RepFair-GAN: Mitigating Representation Bias in GANs Using Gradient Clipping

Fairness has become an essential problem in many domains of Machine Learning (ML), such as classification, natural language processing, and Generative Adversarial Networks (GANs). In this research effort, we study the unfairness of GANs. We formally define a new fairness notion for generative models in terms of the distribution of generated samples sharing the same protected attributes (gender, race, etc.). The defined fairness notion (representational fairness) requires the distribution of the sensitive attributes at the test time to be uniform, and, in particular for GAN model, we show that this fairness notion is violated even when the dataset contains equally represented groups, i.e., the generator favors generating one group of samples over the others at the test time. In this work, we shed light on the source of this representation bias in GANs along with a straightforward method to overcome this problem. We first show on two widely used datasets (MNIST, SVHN) that when the norm of the gradient of one group is more important than the other during the discriminator's training, the generator favours sampling data from one group more than the other at test time. We then show that controlling the groups' gradient norm by performing group-wise gradient norm clipping in the discriminator during the training leads to a more fair data generation in terms of representational fairness compared to existing models while preserving the quality of generated samples.

==> [2022] RepFair-GAN Mitigating Representation Bias in GANs Using Gradient Clipping(2)/images/Vanilla-Gan_avg_magnitude.tex <==
\begin{figure}
\label{fig:average_gradient_magni}
\begin{tikzpicture}
\begin{groupplot}[
  group style={
    group size=1 by 2,
    xlabels at=edge bottom,
    vertical sep=.5cm,
  },
  footnotesize,
  width=\linewidth,
  height=0.55\linewidth,
  dark marker list,
  xmin=0,
  xmax=1,
  xtick=data,
  xlabel={Epochs},
  yticklabel style={%
    /pgf/number format/fixed,
    /pgf/number format/fixed zerofill,
    /pgf/number format/precision=1,
  },
  legend style={
    legend columns=3,
    draw=gray,
    font=\scriptsize,
  },
  legend cell align={left},
  legend pos=north east,
]
\nextgroupplot[
  ymin=.7,
  ymax=.8,
  yticklabel style={%
    /pgf/number format/precision=2,
  },
  ylabel={Accuracy ($\%$)},
]
%\addplot table[x=epoch, y=Accuracy, col sep=comma] {Vanilla-Gan_avg_magnitude.csv};
\nextgroupplot[
  ymin=0,
  ymax=.6,
  ylabel={Fairness ($\%$)},
  legend entries = {avg gradient magnitude for normal images, vg gradient magnitude for shaded},
]
\addplot table[x=epoch, y=normal, col sep=comma] {Vanilla-Gan_avg_magnitude.csv};
\addplot table[x=epoch, y=shaded, col sep=comma] {Vanilla-Gan_avg_magnitude.csv}; 
\end{groupplot}
\end{tikzpicture}
\end{figure}

==> images/Vanilla-Gan_avg_magnitude.tex <==
\begin{figure}
\label{fig:average_gradient_magni}
\begin{tikzpicture}
\begin{groupplot}[
  group style={
    group size=1 by 2,
    xlabels at=edge bottom,
    vertical sep=.5cm,
  },
  footnotesize,
  width=\linewidth,
  height=0.55\linewidth,
  dark marker list,
  xmin=0,
  xmax=1,
  xtick=data,
  xlabel={Epochs},
  yticklabel style={%
    /pgf/number format/fixed,
    /pgf/number format/fixed zerofill,
    /pgf/number format/precision=1,
  },
  legend style={
    legend columns=3,
    draw=gray,
    font=\scriptsize,
  },
  legend cell align={left},
  legend pos=north east,
]
\nextgroupplot[
  ymin=.7,
  ymax=.8,
  yticklabel style={%
    /pgf/number format/precision=2,
  },
  ylabel={Accuracy ($\%$)},
]
%\addplot table[x=epoch, y=Accuracy, col sep=comma] {Vanilla-Gan_avg_magnitude.csv};
\nextgroupplot[
  ymin=0,
  ymax=.6,
  ylabel={Fairness ($\%$)},
  legend entries = {avg gradient magnitude for normal images, vg gradient magnitude for shaded},
]
\addplot table[x=epoch, y=normal, col sep=comma] {Vanilla-Gan_avg_magnitude.csv};
\addplot table[x=epoch, y=shaded, col sep=comma] {Vanilla-Gan_avg_magnitude.csv}; 
\end{groupplot}
\end{tikzpicture}
\end{figure}
